Stress Detection from Photoplethysmography in a Virtual Reality Environment

Personalized virtual reality exposure therapy is a therapeutic practice that can adapt to an individual patient, leading to better health outcomes. Measuring a patient's mental state to adjust the therapy is a critical but difficult task. Most published studies use subjective methods to estimate a patient's mental state, which can be inaccurate. This article proposes a virtual reality exposure therapy (VRET) platform capable of assessing a patient's mental state using non-intrusive and widely available physiological signals such as photoplethysmography (PPG). In a case study, we evaluate how PPG signals can be used to detect two binary classifications: peaceful and stressful states. Sixteen healthy subjects were exposed to the two VR environments (relaxed and stressful). Using LOSO cross-validation, our best classification model could predict the two states with a 70.6% accuracy which outperforms many more complex approaches.

==> Text/5Results.tex <==
%\section{Result}

==> Text/8Acknowledgements.tex <==
\section{Acknowledgements}

==> Text/introduction_old.tex <==
\section{Introduction and Related Work}

Virtual reality (VR) applications provide various experiences by immersing individuals in graphical computer-generated environments. They offer controlled stimuli to induce a particular experience or emotion in the user, e.g., anxiety, stress, relaxation, or presence \cite{halbig2021systematic}. One of the main challenges in VR applications is the possibility of frustration or disengagement of the users due to its excessive simplicity or complexity. Research to date on VR applications has leveraged the user's state evaluation to adapt the difficulty of the games or simulations or activate automated offers for help~\cite{robitaille2019increased}. The user's state evaluation methods come in two main categories: subjective and objective \cite{halbig2021systematic}. In the subjective method, the subjects are explicitly asked to express their own experience through interviews, questionnaires, and think-aloud \cite{greenwald2017investigating}. Although several studies employed the method, they might be biased and break the presence during the experiment \cite{putze2020breaking}. In contrast, the objective method does not need the user to evaluate their experience. Instead, it examines the user's behaviour by direct observation or analysis of physiological data.

Physiological measurements can be collected during exposure fairly unobtrusively and capture sub-conscious states. They provide high-quality quantitative data that can be utilized in Machine Learning (ML) approaches \cite{halbig2021systematic} to predict arousal and valence~\cite{hofmann2018decoding, bilgin2019comparative, ding2020tsception, shumailov2017computational, mavridou2018towards}, anxiety~\cite{hu2018research, wang2018combining, bualan2020investigation, vsalkevicius2019anxiety}, stress~\cite{ishaque2020physiological, ham2017discrimination, cho2017detection, tartarisco2015neuro, robitaille2019increased}, and cognitive workload~\cite{tremmel2019estimating, collins2019measuring, kakkos2019mental, siravenha2019residual}.
Measuring physiological signals is more straightforward because of the easy-to-use wearable sensors' availability~\cite{halbig2021systematic}. 

% There are different use cases of physiological measurements in VR, which come in four main categories: therapy and rehabilitation, training and education, entertainment, and general or functional VR properties \cite{halbig2021systematic}. Physiological measurements in therapy and rehabilitation applications are helpful in assessing the effectiveness of therapy \cite{kothgassner2019virtual, shiban2017diaphragmatic}, adapting the therapeutic system \cite{bualan2020investigation}, and offering appropriate feedback \cite{blum2019heart}. There are two main methods for adapting therapeutic systems: rule-based methods and machine learning approaches. 

% The rule-based studies use a threshold to predict a user's stress or anxiety levels \cite{kritikos2021personalized}, e.g., considering the user's heart rate variability below and more than 100 bpm as a normal and abnormal state \cite{herumurti2019overcoming}. Although these rule-based methods are fast and straightforward, they might not be a good representative of the actual user's state. Therefore, there is a need for more sophisticated techniques like machine learning approaches that automatically find a pattern in physiological signals to predict the user's stress or anxiety level.
Studies show that measuring stress or anxiety is valuable in designing adaptive and personalized VR exposure therapy (VRET) systems, wherein an individual is immersed
in a computer-generated virtual environment to directly confront feared situations or locations that may not be practical or safe to encounter in real life. 
VRET has increasingly been used to treat various anxiety disorders, including specific phobias, e.g., arachnophobia.
Adaptive VRET refines the system's functionalities based on the subject's stress or anxiety. A handful of studies use machine learning methods for stress/anxiety classification in VR, as shown in Tabel~\ref{tab:table1}.

\input{Paper Files/Text/2RelatedWork}

Several stress/anxiety detection studies,~\cite{cho2017detection,ishaque2020physiological,ham2017discrimination,tartarisco2015neuro,robitaille2019increased,ahmad2021multi} in Table~\ref{tab:table1}, used a dynamic or unpredictable virtual environment to induce stress in users, e.g., a roller-coaster ride~\cite{ishaque2020physiological}, or a guard patrolling in a dark and gloomy room~\cite{ham2017discrimination}. These environments are often combined with an additional assignment, e.g., an arithmetic task \cite{cho2017detection} or a Stroop task~\cite{ishaque2020physiological} to further trigger stress in subjects. Although these studies are valuable in predicting stress levels, they do not apply to adaptive VRET, because the type of stress that VRET should be focused on must adversely affect the individuals' quality of life, such as avoiding outdoor activities because of arachnophobia, where spiders may be preset.

% i.e., a therapy technique for treating anxiety disorders in which an individual is gradually exposed to an anxiety source. 

% This is because they induce mental stress~\cite{cho2017detection, ishaque2020physiological} or positive stress~\cite{ishaque2020physiological}, which are usual and necessary to happen to respectively.

Other studies focused on fear of heights~\cite{hu2018research, kaur2019using, wang2018combining, bualan2020investigation, balan2019automatic}, or speech in front of a crowd \cite{vsalkevicius2019anxiety}. Although the studies have focused on valuable types of stress/anxiety for VRET, they mostly used Electroencephalography (EEG), which requires head-mounted sensors that are expensive and intrusive. Instead of using EEG, Salkevicius et al.~\cite{vsalkevicius2019anxiety} suggested using PPG, EDA, and SKT, which are less intrusive. Nevertheless, according to ~\cite{long1982effect}, heart-rate, and blood pressure significantly increase while speaking, suggesting that the changes might not correspond to the amount of stress/anxiety alone. Instead, relaxing/stressful states should be considered in the data collection protocol to make sure changes in physiological measures are mainly associated with anxiety/stress. In addition, the validation method of several studies~\cite{cho2017detection, ishaque2020physiological, ham2017discrimination, robitaille2019increased, hu2018research, wang2018combining, kaur2019using, balan2019automatic, bualan2020investigation} cannot evaluate the system's performance in real-world scenarios. Instead, in order to obtain an independent subject score corresponding to more realistic results for real-life deployment, leave-one-subject-out (LOSO) cross-validation should be applied, i.e., \cite{ahmad2021multi, tartarisco2015neuro, vsalkevicius2019anxiety} in Table~\ref{tab:table1}.

Therefore, estimating subjects' stress/anxiety using physiological signals in scenarios suitable for VRET has remained a challenge. In this study, we design a virtual reality protocol appropriate for VRET to collect a physiological dataset via Photoplethysmography (PPG) biosignal sensor, which is widely available and non-intrusive. The protocol consists of two VR environments, relaxing and stressful. First, we collected the PPG data from sixteen healthy subjects exposed to VR environments. Then we apply classification methods to automatically detect the user's state (relaxed or stressed). The contributions of our work are: 1) developing relaxed and stressful environments for VRET; 2) Applying ML methods to detect stress/anxiety during VR using widely available PPG sensors.


% we used heart rate variability (HRV) to detect stress since previous studies showed that HRV variables changed in response to stress-induced by different methods~\cite{kim2018stress}. HRV can be derived from either ECG or PPG. Although ECG has been used for a long time as the preferred method for measuring HRV, studies showed that estimated HRV based on finger PPG is feasible during rest and mild mental stress~\cite{singstad2021estimation}. PPG can be measured with low-cost, non-invasive and portable methods, i.e., smartwatches \cite{lee2019can}.   

%In the most related research to ours, Mahmoudi-Nejad et al.~\cite{} have proposed a framework for arachnophobia exposure therapy. Their framework adapts the environment based on the users' estimated stress/anxiety level via reinforcement learning. However, the stress estimator in their framework uses an existing real-world dataset. An implication of using such a model is that physiological measures might be affected differently in the VR environments because subjects' reaction depends on the amount of presence and immersiveness of VR environments. In addition, the model requires four separate biosignals, i.e., electrocardiogram (ECG), electrodermal activity (EDA), temperature, and respiration, which are intrusive because they should be attached to different parts of the body.

%Therefore, the application of adaptive VR technology via an accurate stress estimation model for exposure therapy goals has remained a challenge in the literature. In order to address this challenge, we have integrated a VR environment for exposure therapy with a stress estimation model via Photoplethysmography (PPG) biosignal. In this paper, we have developed a relaxed and stressful environment in VR. Sixteen healthy subjects participated in this experiment, wherein we measured the Photoplethysmography (PPG) biosignal. Then we applied classification methods to automatically detect the user's state (relaxed or stressed). The contributions of our work are: 1) developing relaxed and stressful environments in VR; 2) Applying ML methods to detect stress during VR using widely available PPG sensors automatically; 3) developing a stress estimator for adaptive arachnophobia exposure therapy framework.
